Continual Learning to Generalize Forwarding Strategies for Diverse Mobile Wireless Networks

Deep reinforcement learning (DRL) has been successfully used to design forwarding strategies for multi-hop mobile wireless networks. While such strategies can be used directly for networks with varied connectivity and dynamic conditions, developing generalizable approaches that are effective on scenarios significantly different from the training environment remains largely unexplored. In this paper, we propose a framework to address the challenge of generalizability by (i) developing a generalizable base model considering diverse mobile network scenarios, and (ii) using the generalizable base model for new scenarios, and when needed, fine-tuning the base model using a small amount of data from the new scenarios. To support this framework, we first design new features to characterize network variation and feature quality, thereby improving the information used in DRL-based forwarding decisions. We then develop a continual learning (CL) approach able to train DRL models across diverse network scenarios without ``catastrophic forgetting.'' Using extensive evaluation, including real-world scenarios in two cities, we show that our approach is generalizable to unseen mobility scenarios. Compared to a state-of-the-art heuristic forwarding strategy, it leads to up to 78% reduction in delay, 24% improvement in delivery rate, and comparable or slightly higher number of forwards.

==> drl_background.tex <==
\subsection{DRL Background} 
\label{sec:background}

In RL \cite{sutton2018reinforcement}, an agent interacts with its environment to learn a policy, that is, the best action for each state of the environment. A  Markov decision process (MDP) is used to model this policy, defined as a 4-tuple ($\mathcal{S}$, $\mathcal{A}$, $\mathcal{P}$, $\mathcal{R}$) where $\mathcal{S}$ is the set of states, $\mathcal{A}(s)$ are the actions available in each state $s \in \mathcal{S}$, $\mathcal{P}(s,a,s^\prime)$ is a function giving the probability of transitioning from state $s \in \mathcal{S}$ to $s^\prime \in \mathcal{S}$ after taking action $a \in \mathcal{A}$, and $\mathcal{R}(s,a,s^\prime)$ is a function  giving  reward received. In RL, $\mathcal{P}$ and $\mathcal{R}$ are not known but samples can be obtained via interactions with the environment and used to learn a $Q$-value  for each $(s\in \mathcal{S}, a \in \mathcal{A}(s))$ pair.  This Q-value estimates the expected future reward that the RL agent receives after taking action $a$ in state $s$;  the action with the highest $Q$-value is then the  optimal action to take in that state. For large state and action spaces, a deep neural network (DNN) is trained to approximate the mapping from $(s\in \mathcal{S}, a \in \mathcal{A}(s))$ to Q-value, as in DRL, where states and actions are described using feature sets. With  DRL, forwarding decisions are able to easily consider a variety of disparate features. 

Building on the formulation of DRL-based forwarding from \cite{manfredi2024learning}, which we use in our continual learning-based formulation in \S\ref{sec:drl_forwarding}, DRL agents are defined for packets rather than devices to simplify learning. This means that packets themselves choose their next hops rather than devices, and so  features are computed from a packet's viewpoint, while learning tracks  packet states over time. Importantly, this forwarding strategy is able to be trained offline but  be used independently by all packets. The performance of DRL-based routing depends heavily on the input features.  Table \ref{tab:features} lists the set of features used in \cite{manfredi2024learning} as well as the new features (in bold font) that we introduce in this work in the next section (\S\ref{sec:features}). Devices exchange features only with neighbors to limit the control overhead incurred by these exchanges. 

Consider a packet $p$ with destination $d$ that is currently at device $v$ with neighbors $Nbr(v)$.  The {\em state}  for packet $p$ is a set of features defined at different levels of abstraction (packet, direct, indirect) as well as context and neighborhood related features.  Specifically 
$f_{s} (v, p, d) = 
{f}_{packet}(p) \cup 
{f}_{direct}(v, d) \cup 
f_{indirect}(v, d) \cup 
{f}_{nbrhood}(v, d)$. 
Each possible {\em action} for packet $p$,  i.e., forwarding to a neighbor $u \in Nbr(v)$ or keeping it at current device $v$, is then described by the feature set
$f_{a}  (u, p, d) =
{f}_{direct}(u, d) \cup 
f_{indirect}(u, d) \cup
f_{context}(p, u)$.  

We define reward in terms of packet actions: $r_{stay} = -1$ if the packet  stays at its current device,  $r_{transmit} = -2$ if the packet  moves to a neighboring device,  $r_{delivery} = 0$ if the packet reaches its destination, and  $r_{drop} = r_{transmit} / (1-\gamma)$ if the packet is dropped, corresponding to receiving  $r_{transmit}$ for infinite timesteps where $0 \leq \gamma \leq 1$ is the RL discount rate.

As shown in Fig. \ref{fig:multicopy}(a), in our formulation of DRL forwarding, a packet $p$ selects a next hop by separately considering each possible next hop action $u$ for the current state, feeding $f_{s} (v, p, d)$ and $f_{a}  (u, p, d)$ into the trained DNN that encodes the forwarding policy. The DNN outputs a Q-value measuring the goodness of taking action $u$ (that is, having packet $p$ move to $v$'s neighbor device $u$) when in state $f_{s} (v, p, d)$. The action with the highest Q-value is then selected.  In our evaluation, we use a  DNN with 2 fully connected hidden layers with $F$ inputs where $F = |f_{s}(\cdot)| + |f_a(\cdot)|$, $10F$ nodes in the first hidden layer,  $F/2$ nodes in the second hidden layer, and 1 output corresponding to the Q-value for the given state and action pair.


\begin{figure*}[t]%left, bottom, right, top
 \centerline{\hbox{ 
    \subfigure[]
    {\includegraphics[width=2.1in, trim = 18cm 2.3cm 1cm 8.8cm, clip]{figs/multicopy.pdf}}    
    \hspace{0.1in}
    \subfigure[]
    {\includegraphics[width=4.45in, trim = 0.cm 11.4cm 4cm 0.cm, clip]{figs/multicopy.pdf}} 
}}
\vspace{-0.15in}
\caption{{\small (a) Overview the DRL-based forwarding strategy of \cite{wowmom2021-relational,manfredi2023learningarxiv}, and (b) our DRL-based  multi-copy  strategy. \bing{To update.}}}
\vspace{-0.15in}
\label{fig:design-overview}
\end{figure*}

==> large-testing-cases-table.tex <==
\iffalse
\begin{table}[h]
    \centering
    \caption{%Average node degree in large-scale (1000 m $\times$ 1000 m, 100 nodes)  testing scenarios.
    Testing scenarios. All scenarios are for large networks (100 nodes moving in 1000m $\times$ 1000m area), with average node degree for each transmission range ($r=20$, 50 or 80m) shown. In mixed settings, the two numbers indicate the counts of slow and fast nodes, respectively.%in addition to those in Table~\ref{tb:training-cases}. These testing scenarios are
    }
    \begin{tabular}{lcc|ccc}
        \\ \hline %\toprule
        Setting & $N$ & $\bar v$ (m/s) &  $r=20m$ & $r=50m$ & $r=80m$ \\
        \hline
        1-group & 100 & 3 & 1.2 & 6.8 & 15.8 \\ \hline %\midrule
        2-group & 100 & 3 & 1.0 & 5.3 & 12.5 \\ \hline %\midrule
        RWP-3m/s & 100 & 3 & 0.2 & 1.1 & 2.7 \\
        RWP-15m/s & 100 & 15 & 0.2 & 1.1 & 2.7 \\
        RWP-mix1 (20,80) & 100 & 12.6 & 0.2 & 1.1 & 2.7 \\
        RWP-mix2 (50,50) & 100 & 9.0 & 0.2 & 1.1 & 2.7 \\
        RWP-mix3 (80,20) & 100 & 5.4 & 0.2 & 1.0 & 2.7 \\
        \hline %\midrule
        Grid-3m/s & 100 & 3 & 0.1 & 0.6 & 1.8   \\
        Grid-15m/s & 100 & 15 & 0.2 & 0.6 & 1.8 \\
        Grid-mix1 (20,80) & 100 & 12.6 & 0.1 & 0.6 & 1.8 \\
        Grid-mix2 (50,50) & 100 & 9.0 & 0.1 & 0.6 & 1.8  \\
        Grid-mix3 (80,20) & 100 & 5.4& 0.2 & 0.6 & 1.9 \\ 
        \hline %\bottomrule    
    \end{tabular} \label{tb:testing-cases}
\end{table}
\fi


% 20250716 Jin updated the table
\begin{table}[h]
    \centering
    \caption{
    Large-scale testing scenarios:
    100 nodes in 1000m $\times$ 1000m. % area. 
    % (100 nodes moving  in 1000 m $\times$ 1000 m area). 
    % In mixed settings, the two numbers indicate the counts of slow and fast nodes, respectively. }
    }
    \begin{tabular}{lcc|ccc} % <-- Restored the | here for vertical separation
    \hline % <-- Replaced \toprule
    \multirow{2}{*}[-1.5pt]{\textbf{Setting}} & \multirow{2}{*}[-1.5pt]{\textbf{$N$}} & \multirow{2}{*}[-1.5pt]{\textbf{$\bar v$ (m/s)}} & \multicolumn{3}{c}{\textbf{Average node degree}} \\
    \cline{4-6} % <-- Replaced \cmidrule and adjusted span
    & & & $r=20m$ & $r=50m$ & $r=80m$ \\
    \hline % <-- Replaced \midrule
    1-group & 100 & 3.0 & 1.2 & 6.8 & 15.8 \\
    \hline % <-- Replaced \midrule
    2-group & 100 & 3.0 & 1.0 & 5.3 & 12.5 \\
    \hline % <-- Replaced \midrule
    RWP-3m/s & 100 & 3.0 & 0.2 & 1.1 & 2.7 \\
    RWP-15m/s & 100 & 15.0 & 0.2 & 1.1 & 2.7 \\
    RWP-mix1 (20,80) & 100 & 12.6 & 0.2 & 1.1 & 2.7 \\
    RWP-mix2 (50,50) & 100 & 9.0 & 0.2 & 1.1 & 2.7 \\
    RWP-mix3 (80,20) & 100 & 5.4 & 0.2 & 1.0 & 2.7 \\
    \hline % <-- Replaced \midrule
    Grid-3m/s & 100 & 3.0 & 0.1 & 0.6 & 1.8 \\
    Grid-15m/s & 100 & 15.0 & 0.2 & 0.6 & 1.8 \\
    Grid-mix1 (20,80) & 100 & 12.6 & 0.1 & 0.6 & 1.8 \\
    Grid-mix2 (50,50) & 100 & 9.0 & 0.1 & 0.6 & 1.8 \\
    Grid-mix3 (80,20) & 100 & 5.4& 0.2 & 0.6 & 1.9 \\
    \hline % <-- Replaced \bottomrule
\end{tabular} \label{tb:testing-cases}
\parbox{\linewidth}{\footnotesize
    * In mix settings, the \#s of slow and fast nodes are marked in parentheses.}
    % * In mix settings, the two numbers indicate the counts of slow and fast nodes, respectively.}
\end{table}


%wb, split the Manhattan and the two real-world city map, move Manhattan to be an a synthetic trace (since it is not really Manhattan, not actual grid size; not actual movement)
\iffalse 
\begin{table}[h]
    \centering
    \caption{Use case 1 (Manhattan grid topology). \bing{Place holder: fill in average node degree, with one decimal point.}}
    \begin{tabular}{lcccc}
        \\ \hline
        Setting & $N$ & $r=20m$ & $r=50m$ & $r=80m$ \\
        \hline
        Manhattan-3m/s & 100 & 0.1 & 0.6 & 1.8   \\
        Manhattan-15m/s & 100 & 0.2 & 0.6 & 1.8 \\
        Manhattan-mix1 (20,80) & 100 & 0.1 & 0.6 & 1.8 \\
        Manhattan-mix2 (50,50) & 100 & 0.1 & 0.6 & 1.8  \\
        Manhattan-mix3 (80,20) & 100 & 0.2 & 0.6 & 1.9 \\ 
        \hline
    \end{tabular} \label{tb:use-cases-1}
\end{table}
\fi 


==> res-others.tex <==
\subsubsection{Others}
We now consider the best DRL agents obtained from \textsc{gm-train} and \textsc{rwp-train} scenarios, i.e., \textsc{drl-gm} and \textsc{drl-rwp-all}, and evaluate their testing performance. To test whether one DRL agent trained from one mobility model can be applied to another mobility model, we test four combinations by testing each of the \textsc{drl-gm} and  \textsc{drl-rwp-all} agents on each of the \textsc{gm-test}  and \textsc{rwp-test}  scenarios  (see Table \ref{tab:dynamics}). In the following, each point in a plot represents average value  across 5 simulation runs, with  95\% confidence intervals shown. 




\subsubsection{Results for \textsc{gm-test} scenarios}
Fig. \ref{fig:rl-test-results-gm} shows the performance of the DRL agents and the comparison strategies on \textsc{gm-test} when the transmission range $X_{test}$ varies from 20 to 150m. When the transmission range, $X_{test}$, is 20m, all forwarding strategies except Oracle have similar delay  (see Fig. \ref{fig:rl-test-results-gm}(a)); for other transmission ranges, we see significant differences in delay for different strategies. We believe this is  because when $X_{test}=20$m, the network is sufficiently sparse that features are quickly out-of-date  and since all devices are IID and eventually meet each other, there is little intelligent forwarding that can be done.

Unlike Spray\&Wait and Spray\&Focus, the two DRL-based strategies perform consistently  for all transmission ranges. We observe that \textsc{drl-gm} strategy has  the lowest delay except for the Oracle baseline, regardless of $X_{test}$  or number of copies made, as well as some of the smallest maximum queue lengths. Conversely, \textsc{drl-gm}  tends to have many more forwards than \textsc{drl-rwp-all}. \textsc{drl-rwp-all} makes among the fewest forwards of any strategy, only above that of the Oracle (which is not a practical scheme) and Spray-and-Wait strategy (which makes no forwards after the spraying phase). For instance, when $X_{test}$ is 20m, \textsc{drl-rwp-all} performs similarly to Spray\&Wait, i.e., it does not forward packets after the spraying phase, since the network is so sparse and the information is out-of-date, and simply holding a packet until meeting the destination is a good strategy for  both delay and forwards (note the very similar delay of all non-oracle strategies in Fig. \ref{fig:rl-test-results-gm}(a), even those that make many forwards). As $X_{test}$  increases, \textsc{drl-rwp-all} adjusts its behavior by making more forwards than Spray\&Wait, and achieves significantly lower delay. Specifically, when  $X_{test}$  is 150m, the number of forwards of \textsc{drl-rwp-all} becomes close to Spray\&Focus (higher than Spray\&Wait), while achieving significantly lower delay than both Spray\&Focus and Spray\&Wait, indicating that the new temporal features, designed for sparse networks, minimally impact performance when the network is dense.

